Location Attention for Extrapolation to Longer Sequences

Neural networks are surprisingly good at interpolating and perform remarkably well when the training set examples resemble those in the test set. However, they are often unable to extrapolate patterns beyond the seen data, even when the abstractions required for such patterns are simple. In this paper, we first review the notion of extrapolation, why it is important and how one could hope to tackle it. We then focus on a specific type of extrapolation which is especially useful for natural language processing: generalization to sequences that are longer than the training ones. We hypothesize that models with a separate content- and location-based attention are more likely to extrapolate than those with common attention mechanisms. We empirically support our claim for recurrent seq2seq models with our proposed attention on variants of the Lookup Table task. This sheds light on some striking failures of neural models for sequences and on possible methods to approaching such issues.

==> text/background_extrap.tex <==
\section{Related Work}
%\begin{description}
%\item[Robustness] 
%\paragraph{Robustness} Most methods exhibit very high variance when extrapolating \cite{hooker2004diagnostics, weber2018fine}, making them brittle as real world data will not be constrained to $\mathcal{I}_{inter}$. 
%Given a large $\mathcal{D}$ the probability of encountering $\mathbf{x} \in \mathcal{I}_{extra}$ may seem small. 
%However, as noted by \cite{hooker2004diagnostics}, extrapolation is common in practical scenarios as high dimensional problems would typically require an exponentially large $\mathcal{D}$ to be representative and the underlying distribution may vary over time.
%
%\paragraph{Optimization}
%As an infinite number of $f$ would reach the minimum Bayes error in the interpolation setting, the loss function has an infinite amount of minimas making the optimization process hard. 
%This is illustrated by the lack of robustness of neural networks to seemingly minor factors such as the random seed \cite{weber2018fine}, the order in which the examples are shown or the weight updating order \cite{livska2018memorize}. 
%Enforcing extrapolation would create a single global minima corresponding to $t=f$, simplifying the optimisation process \footnote{Similarly to how $L_2$ regularization simplifies the finding of the least squares solution.}.
%
%\paragraph{Abstract Reasoning} 
As neural networks are powerful memorizers  \cite{zhang2016understanding} and easily learn superficial statistical cues \cite{szegedy2013intriguing,jo2017measuring}, testing extrapolation and generalization to samples from the long tails of a distribution %\footnote{Extrapolation as defined we define it, corresponds to testing on samples from the long tails of the distribution rather than samples from an other distribution.} 
might be the only way of quantifying their capacity of abstract reasoning \cite{barrett2018measuring}. 
Methods that are capable of abstract reasoning are key to improve sample efficiency and interpretability as this is reminiscent to how humans learn. 
This argument is well exemplified by \citet{mitchell2018extrapolation}, who state that extrapolation requires exploiting the global structure of a problem similarly to models and equations in physics.
%\end{description}

Given those benefits, one might wonder why so little work has been done in extrapolation. One possible explanation is that the probability of encountering a test example in the extrapolation setting seems low when the training set $\mathcal{D}$ is large.\footnote{Extrapolation is still common in practical scenarios as high dimensional problems would typically require an exponentially large $\mathcal{D}$ to be representative and the underlying distribution may vary over time \cite{hooker2004diagnostics}.} However, such argument fails to consider the possibly high cost of error in an extrapolation setting and how such cost can be a barrier for real-world scenarios that require robustness (e.g. self-driving cars).
%Another possible explanation is the inability of the field of machine learning to operate in such setting \cite{marcus1998rethinking, marcus2018deep}.
%One might even argue that extrapolation is impossible as it is an ill-defined problem.
%While this is true, the same holds for interpolation.
%Yet we are able to build very successful methods for interpolation based on a few key assumptions, typically smoothness of the underlying predictor \cite{domingos2012few}.

%Furthermore, humans extrapolate well beyond the training range \cite{delosh1997extrapolation} thanks to background knowledge and \textbf{inductive biases} \cite{tenenbaum2011grow,lake2017building,feinman2018learning}  which define prior preferences over models \cite{mitchell1980need}.

%The goal is thus to come up with such useful assumptions for extrapolation and incorporate them in our models without constraining their expressivity.


This paper follows recent works that have suggested the importance of extrapolation in Natural Language Processing (NLP).
Recent work by \citet{mitchell2018extrapolation}  have considered using additional constraints to model global structures in language, which they argue to be pivotal for extrapolation.

Our approach is more similar to \citet{weyde2018modelling}, who incorporate an inductive bias for learning identity rules without diminishing the models' expressiveness.
% Specifically, we propose the use of a new location-based attention, which is more prone to extrapolation.
%to impose an inductive bias which is more prone to extrapolate sequences as its inputs and outputs are bounded to be in a given range independent of the sequence length.
% To understand the differences with common attention mechanisms, we first review some of those.
%
%
%[!!!NOTE!!! I don't know where to put the following, but we might get attacked on this if we don't mention it:]
%The only methods that are currently relatively safe to use in an extrapolation setting, are the ones based on Bayesian inference as their predictions in an extrapolation setting will be given highly uncertain. Although this might be the best solution in many cases, we argue that some problems that are easily solvable by humans (such as working with sequences of $n^*=n_{\mathcal{D}}$) should also be solvable by machine learning algorithms.
%
%Furthermore the corollary of this observation, i.e. humans are able to generate and understand infinitely many sentences, mixed with the fact that our experience is finite is the \textit{productive argument} which is often used as a proof of the \textit{principle of compositionality} in semantics \cite{sep-compositionality}.
%
%
%Mitchell et al argue that most scientist view extrapolation as a vital test for the model legitimacy, giving the example Newton's law of gravity. They distinguish current methods based on local smoothing that are only effective in interpolation and models that exploit global structure of the phenomena to be able to extrapolate. They show for example that reversing, which indicates that current model take advantage of statistical regularities in the dataset and do not learn in a human-like manner.


==> text/location.tex <==
In language, it seems crucial to attend to words based on their positions.  
%sequence-to-sequence  frameworks  as  it  has  been  shown  tobe  worst  than  content  one
Location-based attention is not common in sequence-to-sequence frameworks as it has been shown to be worst than content one \cite{luong2015effective}. 
%Indeed, content attention is more general than its location counterpart in an interpolation setting \cite{graves2014neural} as embeddings could learn to encode the location of the word. 
In other frameworks, some models augment content attention to help location addressing by post-processing  \cite{graves2014neural}, by weighting \cite{sukhbaatar2015end} or by adding location queues to the embeddings \cite{vaswani2017attention}.

Many location-attention mechanisms have been proposed in the literature. 
For \textit{seq2seq} models, \citet{luong2015effective} proposed to use Equation \ref{eq:content}, with a score which in independent of the key $\mathbf{w}^T \mathbf{q}_t$ but found no improvement compared to content-attention.
\footnote{ They only considered the interpolation setting, in which content attention is strictly more general than its positional counterpart, as the key and queries can learn to encode their location \cite{graves2014neural}.
%Nevertheless, it is highly improbable that such embedded ``location queues'' would extrapolate to positions not seen during training (see Section \ref{sec:desiderata}).
}
This simple location-based attention does not allow
In  other  frameworks,  some models augment content attention to help location addressing.
The Neural Turing Machine
\cite{graves2014neural}, post-processes the content attention by shifting its location by a number of steps.
Although powerful, it was not designed as an attention mechanism over a sentence and thus does not allow many positional-only patterns such as "attend to the the last word" or "attend to the word in the middle".


